Liouville-Green expansions of exponential form, with an application to modified Bessel functions

Linear second order differential equations of the form $d^{2}w/dz^{2}-\left \{ {u^{2}f\left( u,z\right) +g\left( z\right) }\right\} w=0$ are studied, where $\left| u\right| \rightarrow \infty $ and $z$ lies in a complex bounded or unbounded domain $\mathbf{D}$. If $f\left( u,z\right) $ and $g\left( z\right) $ are meromorphic in $\mathbf{D}$, and $f\left(u,z\right) $ has no zeros, the classical Liouville-Green/WKBJ approximation provides asymptotic expansions involving the exponential function. The coefficients in these expansions either multiply the exponential, or in an alternative form appear in the exponent. The latter case has applications to the simplification of turning point expansions as well as certain quantum mechanic problems, and new computable error bounds are derived. It is shown how these bounds can be sharpened to provide realistic error estimates, and this is illustrated by an application to modified Bessel functions of complex argument and large positive order. Explicit computable error bounds are also derived for asymptotic expansions for particular solutions of the nonhomogeneous equations of the form $d^{2}w/dz^{2}-\left\{ {u^{2}f\left(z\right) +g\left( z\right) }\right\} w=p\left( z\right)$.

==> rsemacros.tex <==
%%
%% This is file `rsemacros.tex'
%% Royal Society of Edinburgh Macros File for Series A Journal
%%
%% Copyright 1998 T&T Productions Ltd
%%
%% Developed by Jonathan Wainwright
%%
%% 19.2.99 `\meas' macro defined
%%
\def\fileversion{v1.02}
\def\filedate{1999/02/19}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%    CONTENTS            %
% ====================== %
% 1. EDITING MACROS      %
% 2. UNITS               %
% 3. MATHS MACROS        %
% 4. GREEK MACROS        %
% 5. FIGURES             %
% 6. SUBEQUATION         %
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%
% EDITING MACROS %
%%%%%%%%%%%%%%%%%%

% \tit  Abbreviation for `\textit'
\newcommand{\tit}[1]{\textit{#1}}

% \tbf  Abbreviation for `\textbf'
\newcommand{\tbf}[1]{\textbf{#1}}

% \tsc  Abbreviation for `\textsc'
\newcommand{\tsc}[1]{\textsc{#1}}

% \mrm  Abbreviation for `\mathrm'
\newcommand{\mrm}[1]{\mathrm{#1}}

% \present Macro for `present address' for use in \author
\newcommand{\present}[1]{\footnote{Present address: #1}}

% \permanent Macro for `permanent address' for use in \author
\newcommand{\permanent}[1]{\footnote{Permanent address: #1}}

% \email Macro for `email address' for use in \affiliation
\newcommand{\email}[1]{{\upshape(\texttt{#1})}}
\newcommand{\twoemails}[2]{{\upshape(\texttt{#1}; \texttt{#2})}}

% \ca   Use only before a number; otherwise use `about',
%       `approximately', etc. - \ca10
%
\newcommand{\ca}{\textit{ca}.\kern1.66pt}

% \et   Omits extra full stop after et al. if at end of sentence,
%       and uses xspace to avoid any unwanted space
%
\makeatletter
\newcommand{\@etalstop}{\ifx\@let@token.%
                          \else.%
                        \fi\xspace}
\newcommand{\etalstop}{\futurelet\@let@token\@etalstop}
\newcommand{\et}{\textit{et al}\etalstop}
\makeatother

% \OK   OK query - prints `OK?' in the margin
%
\newcommand{\OK}[1]{\protect\smash{\underline{#1}}\marginpar{\underline{OK?}}}

% \query   Extended query - prints more detailed query in margin
%
\newcommand{\query}[2]{\protect\smash{\underline{#1}}%
  \marginpar{\small\raggedright#2}}
\newcommand{\gquery}[2]{\query{#1}{#2-\hbox{\raisebox{0.15mm}%
  {$\bigcirc$}\hspace{-2.9mm}\footnotesize{G}}}}

% \mpar   Marginal query for use without underlining text.
%
\newcommand{\mpar}[1]{\marginpar{\small\raggedright#1}}
\newcommand{\empar}[1]{\mpar{\small\raggedright\ \\[-12mm]#1}}

% \press      (In the press.)
% \submitted  (Submitted.)
% \prep       (In preparation.)
% \publ        Publisher?
% \notcited   Not cited in text!
% \details    Details?
% \notinrefs  Not in references!
% \allauthors Provide all authors!
%
\newcommand{\press}{\underline{(In the press.)}\marginpar{\small Details?}}
\newcommand{\submitted}{\underline{(Submitted.)}\marginpar{\small Details?}}
\newcommand{\prep}{\underline{(In preparation.)}\marginpar{\small Details?}}
\newcommand{\publ}{\underline{Publisher.}\marginpar{\small Publisher?}}
\newcommand{\notcited}[1]{\query{#1}{\small Not cited in text!}}
\newcommand{\notinrefs}[1]{\query{#1}{\small Not in References!}}
\newcommand{\allauthors}{\query{\et}{\small Please provide all authors!}}
\newcommand{\details}{\mpar{\small Details?}}
\newcommand{\initials}{\underline{X. X. X.}\marginpar{\small Initials?}}

% \registered   For use after programs such as Adobe Illustrator
%
\newcommand{\registered}{${}^{\bigcirc\hskip-6.4pt\mbox{\tiny R}}$}

% \sect   Section symbol for use only with a section number
%
\newcommand{\sect}{{\usefont{OMS}{cmsy}{m}{n}\S\,}}

% \ns   Natural spacing using \letterspace for use in author names
%
\newcommand{\ns}[1]{\letterspace to 1.15\naturalwidth{#1}}

% \ui   Upright item label
%
\newcommand{\ui}[1]{\item[{\upshape(#1)}]}
\newcommand{\uinp}[1]{\item[{\upshape#1}]}

% \bye  End document
%
\newcommand{\bye}{\label{lastpage}\end{document}}

% \ack  Acknowledgments
%
\newcommand{\ack}{\section*{Acknowledgments}}

% \Issued  For final line
%
\newcommand{\Issued}[1]{\medbreak\centering\footnotesize(\textit{Issued #1})}

\newcommand{\blankoddpage}{\newpage{\thispagestyle{blank}\phantom{blank}}}
\newcommand{\blankevenpage}{\newpage{\thispagestyle{blank}}\cleardoublepage}

% Errata macros
%
\newcommand{\errtitle}[1]{\section*{#1}}
\newcommand{\errauthor}[1]{\centerline{\textsc{By #1}}\bigskip}
\newcommand{\errrefpa}[3]{\centerline{\textit{Proc. R. Soc. Lond.}
A\,\textbf{#1}, #2 (#3)}\bigskip}
\newcommand{\errrefta}[3]{\centerline{\textit{Phil. Trans. R. Soc. Lond.}
A\,\textbf{#1}, #2 (#3)}\bigskip}

%%%%%%%%%%%
%  UNITS  %
%%%%%%%%%%%

% \3   Fixed unbreakable space separating numbers and their units
%      e.g. 5\3cm (no need to group the unit)
%
\newcommand{\3}{\kern2.5pt}

% \C   Degrees Celcius
%      Use in text or math, no need to mbox or add space
%
\newcommand{\C}[1]{\ensuremath{{}^\circ}\textrm{C}\xspace#1}

% \upmu   Upright mu for `micro-' prefix
%
\newcommand{\upmu}[1]{\Pisymbol{psy}{109}#1}

%%%%%%%%%%%%%%%%
% MATHS MACROS %
%%%%%%%%%%%%%%%%

\newcommand{\nn}{\nonumber}
\newcommand{\RE}{R\kern-.667pte}  % Reynolds number
\newcommand{\PR}{P\kern-.667ptr}  % Prandtl number
\newcommand{\NU}{N\kern-.667ptu}  % Nusselt number

\newcommand{\dsty}{\displaystyle}
\newcommand{\ssty}{\scriptstyle}

\newcommand{\link}[1]{\quad\text{#1}\quad} % Linking roman text

% Use AMS binary relations in preference to standard LaTeX symbols
\let\le\leqslant
\let\leq\leqslant
\let\ge\geqslant
\let\geq\geqslant

% `Greater than less than' relation
\newcommand{\gtlt}{\stackrel{\raisebox{2pt}{$\scriptstyle >$}}%
  {\smash{\scriptstyle <}}}

\newcommand{\rd}{\mathrm{d}}            % Roman d for differential
\newcommand{\re}{\mathrm{e}}            % Roman e for exponential
\newcommand{\ri}{\mathrm{i}}            % Roman i for imaginary number
\newcommand{\cc}{\mathrm{c.c.}}         % Abbreviation for `complex conjugate'
\newcommand{\const}{\mathrm{const.}}    % Abbreviation for `constant'

\newcommand{\triup}{\vartriangle}
\newcommand{\tridown}{\triangledown}
\newcommand{\triright}{\vartriangleright}
\newcommand{\trileft}{\vartriangleleft}
\newcommand{\btriup}{\blacktriangle}
\newcommand{\btridown}{\blacktriangledown}
\newcommand{\btriright}{\blacktriangleright}
\newcommand{\btrileft}{\blacktriangleleft}
\newcommand{\bsquare}{{\scriptscriptstyle\blacksquare}}
\newcommand{\blozenge}{\blacklozenge}
\newcommand{\ssquare}{{\scriptscriptstyle\square}}

\DeclareMathOperator{\Real}{Re}  % Real part
\DeclareMathOperator{\Imag}{Im}  % Imaginary part
\DeclareMathOperator{\diag}{diag}         % Diagonal
\DeclareMathOperator{\Int}{Int}           % Integer
\DeclareMathOperator{\Mod}{mod}           % Modulus (de-spaced)
\DeclareMathOperator{\sgn}{sgn}           % Sign
\DeclareMathOperator{\res}{res}           % Residue
\DeclareMathOperator{\Res}{Res}           % Residue
\DeclareMathOperator{\mes}{mes}           % Measure
\DeclareMathOperator{\meas}{meas}         % Measure
\DeclareMathOperator{\erf}{erf}           % Error function
\DeclareMathOperator{\erfc}{erfc}         % Complementary error function
\DeclareMathOperator{\rank}{rank}         % Rank
\DeclareMathOperator{\tr}{tr}             % Trace
\DeclareMathOperator{\Tr}{Tr}             % Trace
\DeclareMathOperator{\Ai}{Ai}             % Airy function
\DeclareMathOperator{\Bi}{Bi}             % Airy function
\DeclareMathOperator{\Ei}{Ei}             %
\DeclareMathOperator{\curl}{curl}         % Curl
\DeclareMathOperator{\grad}{grad}         % Grad
\DeclareMathOperator{\inc}{inc}           % Inc
\DeclareMathOperator{\Hess}{Hess}         % Hessian
\DeclareMathOperator{\arccot}{arccot}     % Inverse cotangent
\DeclareMathOperator{\arcsec}{arcsec}     % Inverse secant
\DeclareMathOperator{\arccosec}{arccosec} % Inverse cosecant
\DeclareMathOperator{\cosec}{cosec}       % Cosecant
\DeclareMathOperator{\sech}{sech}         % Hyperbolic secant
\DeclareMathOperator{\cosech}{cosech}     % Hyperbolic cosecant
\DeclareMathOperator{\arcsinh}{arsinh}    % Inverse hyperbolic sine
\DeclareMathOperator{\arcosh}{arcosh}     % Inverse hyperbolic cosine
\DeclareMathOperator{\artanh}{artanh}     % Inverse hyperbolic tangent
\DeclareMathOperator{\arcoth}{arcoth}     % Inverse hyperbolic cotangent
\DeclareMathOperator{\arsech}{arsech}     % Inverse hyperbolic secant
\DeclareMathOperator{\arcosech}{arcosech} % Inverse hyperbolic cosecant
\DeclareMathOperator{\sn}{sn}             % Jacobian elliptic sinus
\DeclareMathOperator{\cn}{cn}             % Jacobian elliptic cosinus
\DeclareMathOperator{\dn}{dn}             % elliptic functions
\DeclareMathOperator{\supp}{supp}         %
\DeclareMathOperator{\dist}{dist}         %
\DeclareMathOperator{\adj}{adj}           % adjoint
\DeclareMathOperator{\Div}{div}           % divergence
\DeclareMathOperator{\Span}{span}         % span

\newcommand{\dint}{\int\kern-5pt\int}

\newcommand{\qq}{\qquad}

\newcommand{\smfr}[2]{{\textstyle\frac{#1}{#2}}}         % Small fraction
\newcommand{\mdfr}[2]{\hbox{\small$\dsty\frac{#1}{#2}$}}   % Medium fraction

% To display maths inline with a short piece of text left justified
%
\newcommand{\InlineDisplay}[2]{\smallskip\noindent\hbox to \hsize{#1\hfill%
 \begin{math}#2\end{math}\hfill\phantom{#1}}}

% `Frown' accent (upside down \breve, almost!)
%
\newcommand{\frownaccent}[1]{\mathaccent"317F{#1}}

% Bold zero and one
\newcommand{\bzero}{\bm{0}}
\newcommand{\bone}{\bm{1}}
% Phantom zero for use in tables
\newcommand{\0}{\phantom{0}}
% Multicolumn abbreviation
\newcommand{\mc}{\multicolumn}
% Overbrace for use in tables
\newcommand{\ob}[2]{\mc{#1}{c}{$\overbrace{\hspace{#2mm}}$}}
% Smashed vertical brace
\newcommand{\vbrace}[1]{\smash{\left\{ \phantom{\rule{0.1mm}{#1mm}} \right.}}
% Left shift 1st line of an aligned structure
\newcommand{\leftshift}[1]{\hspace{#1mm}&\hspace{-#1mm}}

%%%%%%%%%%%%%%%%
% GREEK MACROS %
%%%%%%%%%%%%%%%%

% Sloping Greek caps
\newcommand{\sDe}{\varDelta}
\newcommand{\sLa}{\varLambda}
\newcommand{\sOm}{\varOmega}
\newcommand{\sSi}{\varSigma}
\newcommand{\sTh}{\varTheta}
\newcommand{\sPh}{\varPhi}
\newcommand{\sPs}{\varPsi}
\newcommand{\sPi}{\varPi}
\newcommand{\sGa}{\varGamma}
\newcommand{\sUp}{\varUpsilon}
\newcommand{\sXi}{\varXi}

% Bold Greek lowercase

\DeclareBoldMathCommand\bal{\alpha}
\DeclareBoldMathCommand\bbe{\beta}
\DeclareBoldMathCommand\bga{\gamma}
\DeclareBoldMathCommand\bde{\delta}
\DeclareBoldMathCommand\bep{\epsilon}
\DeclareBoldMathCommand\bve{\varepsilon}
\DeclareBoldMathCommand\bze{\zeta}
\DeclareBoldMathCommand\bet{\eta}
\DeclareBoldMathCommand\bth{\theta}
\DeclareBoldMathCommand\bio{\iota}
\DeclareBoldMathCommand\bka{\kappa}
\DeclareBoldMathCommand\bla{\lambda}
\DeclareBoldMathCommand\bmu{\mu}
\DeclareBoldMathCommand\bnu{\nu}
\DeclareBoldMathCommand\bxi{\xi}
\DeclareBoldMathCommand\bpi{\pi}
\DeclareBoldMathCommand\brh{\rho}
\DeclareBoldMathCommand\bsi{\sigma}
\DeclareBoldMathCommand\bta{\tau}
\DeclareBoldMathCommand\bup{\upsilon}
\DeclareBoldMathCommand\bph{\phi}
\DeclareBoldMathCommand\bvp{\varphi}
\DeclareBoldMathCommand\bch{\chi}
\DeclareBoldMathCommand\bps{\psi}
\DeclareBoldMathCommand\bom{\omega}

% Bold Greek caps

\DeclareBoldMathCommand\bDe{\varDelta}
\DeclareBoldMathCommand\bLa{\varLambda}
\DeclareBoldMathCommand\bOm{\varOmega}
\DeclareBoldMathCommand\bSi{\varSigma}
\DeclareBoldMathCommand\bTh{\varTheta}
\DeclareBoldMathCommand\bPh{\varPhi}
\DeclareBoldMathCommand\bPs{\varPsi}
\DeclareBoldMathCommand\bPi{\varPi}
\DeclareBoldMathCommand\bGa{\varGamma}
\DeclareBoldMathCommand\bUp{\varUpsilon}
\DeclareBoldMathCommand\bXi{\varXi}

% Greek caps (\Pi, \Xi, \Psi, \Phi not defined)
\newcommand{\De}{\Delta}
\newcommand{\La}{\Lambda}
\newcommand{\Om}{\Omega}
\newcommand{\Si}{\Sigma}
\newcommand{\Th}{\Theta}
\newcommand{\Ga}{\Gamma}
\newcommand{\Up}{\Upsilon}

%%%%%%%%%%%
% FIGURES %
%%%%%%%%%%%

\newcommand{\cfg}[1]{\centerline{\epsfig{file=#1.ps}}}
\newcommand{\cfig}[2]{\centerline{\epsfig{file=#1.ps,width=#2mm}}}
\newcommand{\cefg}[1]{\centerline{\epsfig{file=#1.eps}}}
\newcommand{\cefig}[2]{\centerline{\epsfig{file=#1.eps,width=#2mm}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUBEQUATION ENVIRONMENT %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SUBEQN redefines SUBEQUATIONS to give italic lower case counters

\newenvironment{subeqns}{\begin{subequations}%
  \renewcommand{\theequation}{\theparentequation\,$\alph{equation}$}}%
  {\end{subequations}}

\multlinegap0pt % Removes indent

\endinput
%%
%% End of file `rsemacros.tex'.

